Editing Massive Concepts in Text-to-Image Diffusion Models

Text-to-image diffusion models suffer from the risk of generating outdated, copyrighted, incorrect, and biased content. While previous methods have mitigated the issues on a small scale, it is essential to handle them simultaneously in larger-scale real-world scenarios. We propose a two-stage method, Editing Massive Concepts In Diffusion Models (EMCID). The first stage performs memory optimization for each individual concept with dual self-distillation from text alignment loss and diffusion noise prediction loss. The second stage conducts massive concept editing with multi-layer, closed form model editing. We further propose a comprehensive benchmark, named ImageNet Concept Editing Benchmark (ICEB), for evaluating massive concept editing for T2I models with two subtasks, free-form prompts, massive concept categories, and extensive evaluation metrics. Extensive experiments conducted on our proposed benchmark and previous benchmarks demonstrate the superior scalability of EMCID for editing up to 1,000 concepts, providing a practical approach for fast adjustment and re-deployment of T2I diffusion models in real-world applications.

==> figure_latex/GreatWave.tex <==
\begin{figure*}[ht!]
\vspace{-1em}
    \centering    
    \includegraphics[width=\linewidth]{figure_src/GreatWave.jpg}
    \vspace{-0.30in}
    \caption{
    Our method demonstrates effective preservation of the holdout artist style even after extensive concept editing. In comparison to UCE~(top row), our method~(bottom row) successfully maintains the holdout artist style of ``The Great Wave off Kanagawa'' even when erasing 1000 artist styles.
    }
    \label{fig:greatwave}
\end{figure*}

==> figure_latex/aiced_summary_30.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure_src/aiced_summary_max-30.pdf}
    \caption{
    We test all existing concept editing methods for T2I diffusion models on the task of Arbitrary Concept Editing, for editing up to 30 concepts. Our method presents both exceptional generalization abilities and specificity. 
    }
    \label{fig:aiced_30}
\end{figure*}

==> figure_latex/artists_coco_eval.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figure_src/artists_coco_eval.pdf}
    \vspace{-0.30in}
    \caption{
    Above we showcase the preservation of the generation capabilities after erasing up to 1,000 artist styles, evaluated on COCO-30k prompts. In contrast to the baseline method, our method hardly contaminates the model's general performances even after erasing up to 1,000 artist styles.
    }
    \label{fig:artists_coco}
\end{figure}

==> figure_latex/main_fig.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle%
\vspace{-0.3in}%
\begin{center}
    \centering\includegraphics[width=\linewidth]{figure_src/main_fig_v2.pdf}
        \vspace{-0.30in}
        \captionof{figure}{
        % \enze{caption too short}
        Our method \method{} generally edits \textbf{target concepts}, the concepts intended to be modified, to match \textbf{anchor concepts}, the concepts towards which target concepts are to be altered. 
        Our method can update, forget, rectify, and debias various concepts simultaneously at a large scale. 
        }
        \label{fig:mainfig}
\end{center}
}]

==> figure_latex/problem_setup.tex <==
\begin{figure*}
\vspace{-0.2in}
    \centering
\includegraphics[width=0.9\linewidth]{figure_src/problem_setup.pdf}
    \vspace{-0.1in}
    \caption{
    Our task formulation unifies various concept editing tasks. We present an example for each task.
      } 
    \vspace{-0.2in}
    \label{fig:problem setup}
    
\end{figure*}

==> figure_latex/supp_rectification_qualitative.tex <==
\begin{figure*}[ht]
\vspace{-1em}
    \centering    
    \includegraphics[width=\linewidth]{figure_src/rectification_qualitative.pdf}
    \vspace{-0.30in}
    \caption{
    We demonstrate more examples for the task of Concept Rectification and further compare \method{} with UCE. The 7 misunderstood aliases are rectified simultaneously with UCE and \method{} separately. Our method~(fourth row) can constantly rectify the misunderstood aliases of concepts, while UCE~(third row) often fails to succeed.
    }
    \label{fig:more rectification}
\end{figure*}

==> figure_latex/the_starry_night.tex <==
\begin{figure*}[ht!]
\vspace{-1em}
    \centering    
    \includegraphics[width=\linewidth]{figure_src/forget starry night.jpg}
    \vspace{-0.30in}
    \caption{We demonstrate the performance of our method in terms of erasing artist style under various editing intensity $\alpha$. We present the generated images under varying editing intensity $\alpha$ by erasing the concepts of ``Van Gogh'' and ``The Starry Night''. The top row corresponds to the prompt ``The Starry Night by Vincent van Gogh'' and illustrates the gradual fading of the artwork ``The Starry Night'' as the editing intensity $\alpha$ increases. The bottom row corresponds to the prompt ``Girl with a Pearl Earring by Johannes Vermeer''. Even with the increasing editing intensity, our method retains concepts of another artist's style ~(Johannes Vermeer).
     }
    \label{fig:starry night}
\end{figure*}

==> tables/erase_artsits_coco.tex <==
\begin{table*}
\centering
    \begin{subtable}{0.4\linewidth}
        \begin{tabular}{lccc}
            \textbf{\# Concepts} & \textbf{CLIP $\uparrow$}  & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} \tabularnewline
             \hline
             5  & 26.25 & 0.08 & 14.31 \tabularnewline
             10  & 26.31 & 0.13 & 15.57  \tabularnewline
             50 & 26.06 & 0.22 &  15.11 \tabularnewline
             100  & 25.11 & 0.30 &  15.11 \tabularnewline
             500  & 18.14 & 0.44 & 72.41 \tabularnewline
             1000 & 15.41 & 0.48 & 85.45 \tabularnewline
             \hdashline
             Original SD & 26.62 & - & 13.93 \tabularnewline
        \end{tabular}
        \caption{
         UCE
        }
    \end{subtable}
    \begin{subtable}{0.4\linewidth}
        \begin{tabular}{lccc}
        \textbf{\# Concepts} & \textbf{CLIP $\uparrow$}  & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} \tabularnewline
         \hline
         5 & 26.62 & 0.01 &  13.94 \tabularnewline
         10 & 26.62 & 0.02 &  14.02 \tabularnewline
         50 & 26.61 & 0.03 &  14.00 \tabularnewline
         100  & 26.60 & 0.04 &  14.00 \tabularnewline
         500  & 26.58 & 0.06 & 14.28 \tabularnewline
         1000 & 26.53 & 0.07 & 14.21 \tabularnewline
         \hdashline
         Original SD & 26.62 & - & 13.93 \tabularnewline
    \end{tabular}
        \caption{
        \method{}(ours)
        }
    \end{subtable}
    \caption{More detailed COCO results}
\end{table*}

